DualPrim: Compact 3D Reconstruction with Positive and Negative Primitives

Neural reconstructions often trade structure for fidelity, yielding dense and unstructured meshes with irregular topology and weak part boundaries that hinder editing, animation, and downstream asset reuse. We present DualPrim, a compact and structured 3D reconstruction framework. Unlike additive-only implicit or primitive methods, DualPrim represents shapes with positive and negative superquadrics: the former builds the bases while the latter carves local volumes through a differentiable operator, enabling topology-aware modeling of holes and concavities. This additive-subtractive design increases the representational power without sacrificing compactness or differentiability. We embed DualPrim in a volumetric differentiable renderer, enabling end-to-end learning from multi-view images and seamless mesh export via closed-form boolean difference. Empirically, DualPrim delivers state-of-the-art accuracy and produces compact, structured, and interpretable outputs that better satisfy downstream needs than additive-only alternatives.

==> figures/comparison_itw.tex <==
\renewcommand{\arraystretch}{1.1}
\newcommand{\itwImgWidth}{0.13}
\setlength{\tabcolsep}{2pt}

% --------------------------------------------------
% Macro for one image
% --------------------------------------------------
\newcommand{\itwimg}[2][]{%
  \vbox{%
    \hbox{\includegraphics[width=\itwImgWidth\textwidth]{#2}}%
    \ifx&#1&%
      % do nothing if #1 is empty
    \else
      % \vskip 1mm
      \vspace{-2mm}
      \hbox to \itwImgWidth\textwidth{\hss\small #1\hss}%
    \fi
  }%
}
% --------------------------------------------------
% Macro for one object (two rows)
% args:
% 1 object folder name
% 2 object name prefix
% 3 view id
% --------------------------------------------------
\newcommand{\tworowobjitw}[3]{

% ---- first row ----
\itwimg[Input]{figures/itw_renderings/row0_thumbnail/#2_26views_input.png} &
\itwimg[Ours]{figures/itw_renderings/renderings_#1/#2_ours_view_#3.png} &
\itwimg[PA~\cite{ye2025primitiveanything}]{figures/itw_renderings/renderings_#1/#2_pa_view_#3.png} &
\itwimg[MA~\cite{chen2024meshanything}]{figures/itw_renderings/renderings_#1/#2_meshanything_view_#3.png} &
\itwimg[MP~\cite{Liu2023marching}]{figures/itw_renderings/renderings_#1/#2_mp_view_#3.png} &
\itwimg[EMS~\cite{liu2022EMS}]{figures/itw_renderings/renderings_#1/#2_ems_view_#3.png} &
\itwimg[NVD~\cite{Munkberg_2022_CVPR}]{figures/itw_renderings/renderings_#1/#2_nvdiffrec_view_#3.png}
\vspace{-2mm}
\\

% ---- second row ----
\itwimg[FC~\cite{shen2023flexicubes}]{figures/itw_renderings/renderings_#1/#2_flexicube_view_#3.png} &
\itwimg[RNS~\cite{rnbneus}]{figures/itw_renderings/renderings_#1/#2_neus2_view_#3.png} &
\itwimg[{CAPRI}~\cite{yu2022capri}]{figures/itw_renderings/renderings_#1/#2_capri_view_#3.png} &
\itwimg[{D$^{2}$CSG}~\cite{yu2023d}]{figures/itw_renderings/renderings_#1/#2_d2csg_view_#3.png} &
\itwimg[{DiffCSG}~\cite{yuan2024diffcsg}]{figures/itw_renderings/renderings_#1/#2_diffcsg_view_#3.png} &
\itwimg[2DGS~\cite{huang20242dgs}+MC]{figures/itw_renderings/renderings_#1/#2_2dgs_view_#3.png} &
\itwimg[2DGS~\cite{huang20242dgs}+CSG~\cite{yu2022capri}]{figures/itw_renderings/renderings_#1/#2_2dgs_csg_view_#3.png}
\vspace{-2mm} \\[2pt]
}

\begin{figure*}[t]
\centering

\begin{tabular}{c c c c c c c}

% --------------------------------------------------
% Objects
% --------------------------------------------------

\tworowobjitw{judy_hopps_v3}{judy_hopps_v3}{016}
\vspace{-3mm}
\tworowobjitw{mario_-_super_mario_odyssey_rigged}{mario_-_super_mario_odyssey_rigged}{016}
\vspace{-3mm}
% \tworowobjitw{pikachu_with_cake_M}{pikachu_with_cake_M}{016}
% \vspace{-3mm}
\tworowobjitw{sharkbite_2s_great_white_shark}{sharkbite_2s_great_white_shark}{018}
\vspace{-3mm}
\tworowobjitw{shiba}{shiba}{029}
\vspace{-3mm}
\tworowobjitw{usagi_chiikawa}{usagi_chiikawa}{022}

\end{tabular}

\caption{
Qualitative comparison on in-the-wild objects.
Each object occupies two rows.
The first row shows input, Ours, PA, MA, MP, EMS, and NVD.
The second row shows FC, RNS, CAPRI, D$^{2}$CSG, DiffCSG, 2DGS+MC, and 2DGS+CSG.
}
\label{fig:supp_comparison_itw}
\end{figure*}

==> figures/supp_comparison_cvpr2026.tex <==
\renewcommand{\arraystretch}{1.1}
\newcommand{\suppImgWidth}{0.10}
\setlength{\tabcolsep}{10pt}

% --------------------------------------------------
% Macro for one image
% --------------------------------------------------
% \newcommand{\itwimg}[1]{\includegraphics[width=\itwImgWidth\textwidth]{#1}}
\newcommand{\suppImg}[2][]{%
  \vbox{%
    \hbox{\includegraphics[width=\suppImgWidth\textwidth]{figures/shapenet/#2}}%
    \ifx &#1&%
      % do nothing if #1 is empty
    \else
      % \vskip 1mm
      \hbox to \suppImgWidth\textwidth{\hss\small #1\hss}%
    \fi
  }%
}
% --------------------------------------------------
% Macro for one object (two rows)
% args:
% 1 object folder name
% 2 object name prefix
% 3 view id
% --------------------------------------------------
\newcommand{\tworowobjsupp}[2]{

% ---- first row ----
\suppImg[Input]{#1_input.png} &
\suppImg[Ours]{#2_#1_ours.png} &
\suppImg[PA~\cite{ye2025primitiveanything}]{#2_#1_pa.png} &
\suppImg[MA~\cite{chen2024meshanything}]{#2_#1_ma.png} &
\suppImg[MP~\cite{Liu2023marching}]{#2_#1_mp.png} &
\suppImg[EMS~\cite{liu2022EMS}]{#2_#1_ems.png} &
\suppImg[NVD~\cite{Munkberg_2022_CVPR}]{#2_#1_nvdiffrec.png}
\\

% ---- second row ----
\suppImg[FC~\cite{shen2023flexicubes}]{#2_#1_flexicube.png} &
\suppImg[RNS~\cite{rnbneus}]{#2_#1_neus2.png} &
\suppImg[{CAPRI}~\cite{yu2022capri}]{#2_#1_capri.png} &
\suppImg[{D$^{2}$CSG}~\cite{yu2023d}]{#2_#1_d2csg.png} &
\suppImg[{DiffCSG}~\cite{yuan2024diffcsg}]{#2_#1_diffcsg.png} &
\suppImg[2DGS~\cite{huang20242dgs}+MC]{#2_#1_2dgs_mc.png} &
\suppImg[2DGS~\cite{huang20242dgs}+CSG~\cite{yu2022capri}]{#2_#1_2dgs_csg.png}
\vspace{-1mm} \\[2pt]
}

\begin{figure*}[t]
\centering

\begin{tabular}{c c c c c c c}

% --------------------------------------------------
% Objects
% --------------------------------------------------

\tworowobjsupp{12f3fb99c95c6a7357891d676f728bc0}{airplane}
\vspace{-3mm}
\tworowobjsupp{10cfa696ba2259ccbbba142d6df53ce}{bench}
\vspace{-3mm}
\tworowobjsupp{2d1aa4e124c0dd5bf937e5c6aa3f9597}{bottle}
\vspace{-3mm}
\tworowobjsupp{1db4071178f5818250da8b99982a3057}{faucet}
\vspace{-3mm}
\tworowobjsupp{2b326c82b14dcdcfaf0affed7cfb91de}{clock}
\vspace{-3mm}
\tworowobjsupp{13e1e13465fa1a67b362845c6edb57fc}{faucet}

\end{tabular}

\caption{
Qualitative comparison on ShapeNet objects (part 1).
Each object occupies two rows.
The first row shows input, Ours, PA, MA, MP, EMS, and NVD.
The second row shows FC, RNS, CAPRI, D$^{2}$CSG, DiffCSG, 2DGS+MC, and 2DGS+CSG.
}
\label{fig:supp_comparison_cvpr2026_1}
\end{figure*}



\begin{figure*}[t]
\centering

\begin{tabular}{c c c c c c c}

% --------------------------------------------------
% Objects
% --------------------------------------------------

\tworowobjsupp{29def96b77d4cfe372f9a9353d57f9ef}{table}
\vspace{-3mm}
\tworowobjsupp{1309cb5bbd90c7b250da8b99982a3057}{faucet}
\vspace{-3mm}
\tworowobjsupp{5b39e6a8f57199409bda39e34f423da8}{bookshelf}
\vspace{-3mm}
\tworowobjsupp{15e38eb29fb84898e7e684d25d4dcaf0}{lamp}
\vspace{-3mm}
\tworowobjsupp{18a9c13c3999e9c186abe5555a3b447d}{table}
\end{tabular}

\caption{
Qualitative comparison on ShapeNet objects (part 2).
Each object occupies two rows.
The first row shows input, Ours, PA, MA, MP, EMS, and NVD.
The second row shows FC, RNS, CAPRI, D$^{2}$CSG, DiffCSG, 2DGS+MC, and 2DGS+CSG.
}
\label{fig:supp_comparison_cvpr2026_2}
\end{figure*}

==> tables/primitive_init.tex <==

\begin{table}[t]
    \centering
    \vspace{-4mm}
    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Parameter Name} & \textbf{Shape} & \textbf{Init Value} \\
        \hline
        $(a_{x}, a_{y}, a_{z})$ & $(2, 3)$ & $0.1$\\
        \hline
        $(\epsa, \epsb)$ & $(2, 2)$ & $1.0$\\
        \hline
        $\transparency$ & $(1)$  & $1.0$\\
        \hline
        $\sharpness$ & $(1)$& $0.5$\\
        \hline
        $\trans$ & $(2, 3)$& $U(0, 1)$\\
        \hline
        $\rot$ & $(2, 3)$& $1$\\
        \hline
        basic color $\cbasic$ & $(3)$ & $U(0, 1)$\\
        \hline
    \end{tabular}
    \caption{The initial super-primitive parameter values for \MethodNameShort.}
    \vspace{-2mm}
    \label{table:primitive_init}
\end{table}

